FurnitureBench: Reproducible Real-World Benchmark for Long-Horizon Complex Manipulation

Reinforcement learning (RL), imitation learning (IL), and task and motion planning (TAMP) have demonstrated impressive performance across various robotic manipulation tasks. However, these approaches have been limited to learning simple behaviors in current real-world manipulation benchmarks, such as pushing or pick-and-place. To enable more complex, long-horizon behaviors of an autonomous robot, we propose to focus on real-world furniture assembly, a complex, long-horizon robot manipulation task that requires addressing many current robotic manipulation challenges to solve. We present FurnitureBench, a reproducible real-world furniture assembly benchmark aimed at providing a low barrier for entry and being easily reproducible, so that researchers across the world can reliably test their algorithms and compare them against prior work. For ease of use, we provide 200+ hours of pre-collected data (5000+ demonstrations), 3D printable furniture models, a robotic environment setup guide, and systematic task initialization. Furthermore, we provide FurnitureSim, a fast and realistic simulator of FurnitureBench. We benchmark the performance of offline RL and IL algorithms on our assembly tasks and demonstrate the need to improve such algorithms to be able to solve our tasks in the real world, providing ample opportunities for future research.

==> table/bc_hyperparams.tex <==
\begin{table}[ht]
  \caption{BC hyperparameters.}
  \label{tab:hyperparameter_bc}
  \centering
  \begin{tabular}{ll}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Learning rate & 3e-4 \\ 
    Learning rate decay & Step decay \\
    Learning rate decay factor & 0.5 \\
    \# Mini-batches & 64 \\
    \# Hidden units &(512, 256, 256)  \\
    Activation & ReLU  \\
    Image encoder & R3M, VIP, ResNet-18 \\
    % Action normalization & True \\
    \bottomrule
  \end{tabular}
\end{table}

==> table/evaluation_all.tex <==
\begin{table*}[ht]
\centering
\caption{Full-assembly and single-skill benchmark results. \yw{numbers are random, can be a bar chart}}
\label{tab:evaluation_all}
\begin{tabular}{l|cc|ccccc|cccc}
    \toprule
     & \multicolumn{2}{c|}{Full-Assembly Benchmark} & \multicolumn{5}{c|}{Single-Skill Benchmark (First 5 Skills)} & \multicolumn{4}{c}{Skill Composition} \\
    % \midrule
    %  & Avg. Phases & Best Phases & Grasping~1 & Placing & Grasping~2 & Inserting & Screwing & 1-5 & 2-5 & 3-5 & 4-5 \\
     & Avg. Phases & Best Phases & Skill 1 & Skill 2 & Skill 3 & Skill 4 & Skill 5 & 1-5 & 2-5 & 3-5 & 4-5 \\
    % \midrule
    % \multicolumn{6}{c}{\texttt{one\_leg}} \\
    % \midrule
    % % \texttt{one\_leg}          &       &       &       &       \\
    % BC                              &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 \\
    % IQL                             &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 \\
    \midrule
    %\multicolumn{12}{c}{\texttt{lamp}} \\
    \multicolumn{3}{l|}{\texttt{lamp}} & Grasping~1 & Placing & Grasping~2 & Inserting & Screwing & & & \\
    \midrule
    % \texttt{lamp}              &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5\\
    IQL                             & 0.15 & 0.18 &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \midrule
    % \multicolumn{12}{c}{\texttt{square\_table}} \\
    \multicolumn{3}{l|}{\texttt{square\_table}} &  &  &  &  &  & & & \\
    \midrule
    % \texttt{square\_table}     &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 0.95 & 0.10  & 0.10  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    IQL                             & 0.15 & 0.18 &  0.90 & 0.95 & 0.10  & 0.10  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \midrule
    % \multicolumn{12}{c}{\texttt{desk}} \\
    \multicolumn{3}{l|}{\texttt{desk}} &  & &  &  & & & & \\
    \midrule
    % \texttt{desk}              &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 0.91 & 0.09  & 0.20  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    IQL                             & 0.15 & 0.18 &  0.90 & 0.91 & 0.09  & 0.20  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \midrule
    % \multicolumn{12}{c}{\texttt{round\_table}} \\
    \multicolumn{3}{l|}{\texttt{round\_table}} &  &  &  &  & & & & \\
    \midrule
    % \texttt{round\_table}      &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 0.91 & 0.16  & 0.30  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    IQL                             & 0.15 & 0.18 &  0.90 & 0.91 & 0.16  & 0.30  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \midrule
    % \multicolumn{12}{c}{\texttt{stool}} \\
    \multicolumn{3}{l|}{\texttt{stool}} &  &  &  & & & & & \\
    \midrule
    % \texttt{stool}             &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 0.84 & 0.09  & 0.14  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    IQL                             & 0.15 & 0.18 &  0.90 & 0.84 & 0.09  & 0.14  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \midrule
    % \multicolumn{12}{c}{\texttt{chair}} \\
    \multicolumn{3}{l|}{\texttt{chair}} &  &  &  &  &  & & & \\
    \midrule
    % \texttt{chair}             &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 0.76 & 0.07  & 0.15  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    IQL                             & 0.15 & 0.18 &  0.90 & 0.76 & 0.07  & 0.15  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \midrule
    % \multicolumn{12}{c}{\texttt{drawer}} \\
    \multicolumn{3}{l|}{\texttt{drawer}} & Grasping~1 & Placing & Grasping~2 & Inserting & Pushing & & & \\
    \midrule
    % \texttt{drawer}            &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 1.00 & 0.13  & 0.13  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    IQL                             & 0.15 & 0.18 &  0.90 & 1.00 & 0.13  & 0.13  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \midrule
    % \multicolumn{12}{c}{\texttt{cabinet}} \\
    \multicolumn{3}{l|}{\texttt{cabinet}} & Grasping~1 & Inserting & Grasping~2 & Inserting & Flipping & & & \\
    \midrule
    % \texttt{cabinet}           &       &       &       &       \\
    BC                              & 0.15 & 0.18 &  0.90 & 0.97 & 0.04  & 0.26  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    IQL                             & 0.15 & 0.18 &  0.90 & 0.97 & 0.04  & 0.26  & 0.15 &  0.8 & 0.7 & 0.6 & 0.5 \\
    \bottomrule
\end{tabular}
\end{table*}

==> table/evaluation_all_fulltask.tex <==
\begin{table}[ht]
\centering
\caption{Results on all furniture models. \yw{numbers are random}}
\label{tab:evaluation_all_fulltask}
\begin{tabular}{ll|cc}
    \toprule
    & & Average phases & Best phases \\
    \midrule
    \multirow{2}{*}{\texttt{lamp}}              &  BC   & 0.15  & 0.18   \\
                                                &  IQL  & 0.15  & 0.18   \\
    \midrule
    \multirow{2}{*}{\texttt{square\_table}}     &  BC   & 0.10  & 0.10   \\
                                                &  IQL  & 0.10  & 0.10   \\
    \midrule
    \multirow{2}{*}{\texttt{desk}}              &  BC   & 0.09  & 0.20   \\
                                                &  IQL  & 0.09  & 0.20   \\
    \midrule
    \multirow{2}{*}{\texttt{drawer}}            &  BC   & 0.13  & 0.13   \\
                                                &  IQL  & 0.13  & 0.13   \\
    \midrule
    \multirow{2}{*}{\texttt{cabinet}}           &  BC   & 0.04  & 0.26   \\
                                                &  IQL  & 0.04  & 0.26   \\
    \midrule
    \multirow{2}{*}{\texttt{round\_table}}      &  BC   & 0.16  & 0.30   \\
                                                &  IQL  & 0.16  & 0.30   \\
    \midrule
    \multirow{2}{*}{\texttt{stool}}             &  BC   & 0.09  & 0.14   \\
                                                &  IQL  & 0.09  & 0.14   \\
    \midrule
    \multirow{2}{*}{\texttt{chair}}             &  BC   & 0.07  & 0.15   \\
                                                &  IQL  & 0.07  & 0.15   \\
    \bottomrule
\end{tabular}
\end{table}

==> table/evaluation_all_simulation.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/simulation_performance.pdf}
%     \label{fig:simulation_performance}
% \end{figure}

\begin{table}[ht]
\centering
\caption{Simulated results on all furniture models.}
\label{tab:evaluation_all_fulltask_simulation}
\begin{tabular}{ll|cc}
    \toprule
    & & Average phases & Best phases \\
    \midrule
    \multirow{2}{*}{\texttt{lamp}}              &  BC   & 0.15  & 0.18   \\
                                                &  IQL  & 0.15  & 0.18   \\
    \midrule
    \multirow{2}{*}{\texttt{square\_table}}     &  BC   & 0.10  & 0.10   \\
                                                &  IQL  & 0.10  & 0.10   \\
    \midrule
    \multirow{2}{*}{\texttt{desk}}              &  BC   & 0.09  & 0.20   \\
                                                &  IQL  & 0.09  & 0.20   \\
    \midrule
    \multirow{2}{*}{\texttt{drawer}}            &  BC   & 0.13  & 0.13   \\
                                                &  IQL  & 0.13  & 0.13   \\
    \midrule
    \multirow{2}{*}{\texttt{cabinet}}           &  BC   & 0.04  & 0.26   \\
                                                &  IQL  & 0.04  & 0.26   \\
    \midrule
    \multirow{2}{*}{\texttt{round\_table}}      &  BC   & 0.16  & 0.30   \\
                                                &  IQL  & 0.16  & 0.30   \\
    \midrule
    \multirow{2}{*}{\texttt{stool}}             &  BC   & 0.09  & 0.14   \\
                                                &  IQL  & 0.09  & 0.14   \\
    \midrule
    \multirow{2}{*}{\texttt{chair}}             &  BC   & 0.07  & 0.15   \\
                                                &  IQL  & 0.07  & 0.15   \\
    \bottomrule
\end{tabular}
\end{table}

==> table/evaluation_all_subtask.tex <==
\begin{table}[ht]
\centering
\caption{Subtask success rates of all furniture models. \yw{numbers are random, can be a bar chart}}
\label{tab:evaluation_all_subtask}
\begin{tabular}{l|ccccc}
    \toprule
    Method & Grasping~1 & Placing & Grasping~2 & Inserting & Screwing \\
    % \midrule
    % \multicolumn{6}{c}{\texttt{one\_leg}} \\
    % \midrule
    % % \texttt{one\_leg}          &       &       &       &       \\
    % BC                              &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 \\
    % IQL                             &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{lamp}} \\
    \midrule
    % \texttt{lamp}              &       &       &       &       \\
    BC                              &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 \\
    IQL                             &  0.90 & 0.92 & 0.15  & 0.18  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{square\_table}} \\
    \midrule
    % \texttt{square\_table}     &       &       &       &       \\
    BC                              &  0.90 & 0.95 & 0.10  & 0.10  & 0.15 \\
    IQL                             &  0.90 & 0.95 & 0.10  & 0.10  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{desk}} \\
    \midrule
    % \texttt{desk}              &       &       &       &       \\
    BC                              &  0.90 & 0.91 & 0.09  & 0.20  & 0.15 \\
    IQL                             &  0.90 & 0.91 & 0.09  & 0.20  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{drawer}} \\
    \midrule
    % \texttt{drawer}            &       &       &       &       \\
    BC                              &  0.90 & 1.00 & 0.13  & 0.13  & 0.15 \\
    IQL                             &  0.90 & 1.00 & 0.13  & 0.13  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{cabinet}} \\
    \midrule
    % \texttt{cabinet}           &       &       &       &       \\
    BC                              &  0.90 & 0.97 & 0.04  & 0.26  & 0.15 \\
    IQL                             &  0.90 & 0.97 & 0.04  & 0.26  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{round\_table}} \\
    \midrule
    % \texttt{round\_table}      &       &       &       &       \\
    BC                              &  0.90 & 0.91 & 0.16  & 0.30  & 0.15 \\
    IQL                             &  0.90 & 0.91 & 0.16  & 0.30  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{stool}} \\
    \midrule
    % \texttt{stool}             &       &       &       &       \\
    BC                              &  0.90 & 0.84 & 0.09  & 0.14  & 0.15 \\
    IQL                             &  0.90 & 0.84 & 0.09  & 0.14  & 0.15 \\
    \midrule
    \multicolumn{6}{c}{\texttt{chair}} \\
    \midrule
    % \texttt{chair}             &       &       &       &       \\
    BC                              &  0.90 & 0.76 & 0.07  & 0.15  & 0.15 \\
    IQL                             &  0.90 & 0.76 & 0.07  & 0.15  & 0.15 \\
    \bottomrule
\end{tabular}
\end{table}

==> table/evaluation_one_leg_fulltask.tex <==
\begin{table}[ht]
\centering
\caption{
    Results on the one-leg assembly task.
    % Average phases over 10 evaluation runs with variations of the baselines and different number of demonstrations. The numbers in the parentheses mean the best completed phase among 10 evaluation runs.
}
\label{tab:evaluation_one_leg_fulltask}    
\begin{tabular}{l|c|c|c}
    \toprule
    Viewpoint & Fixed & Variable & Fixed\,+\,Variable \\
    \midrule
        & 500 demos & 400 demos  & 500\,+\,400 demos   \\
    \midrule
    IQL & \textbf{0.20 (0.33)} & \textbf{0.55 (0.67)}    & \textbf{0.73 (1.00)} \\
    BC  & 0 (0) &  0.47 (0.67)  &  0.53 (0.67) \\
    IRIS & 0.08 (0.33) & 0.53 (0.67) & 0.52 (0.67) \\
    \bottomrule
\end{tabular}
% \begin{tabular}{l|c|cccc|c}
%     \toprule
%     Viewpoint & \textbf{Fixed} & \multicolumn{4}{c}{\textbf{Variable}} & \textbf{Mixed} \\
%     \midrule
%                     & 500 demos & 100 demos  & 200 demos     & 300 demos  &  400 demos  & 500 + 400 demos   \\
%     \midrule
%     IQL & 0.20 (0.33) &  0.33 (0.50)        & 0.18 (0.50)            & 0.43 (0.67)       &  \textbf{0.55 (0.67)}                 &  \textbf{0.73 (1.00)} \\
%     %IQL w/ dropout  & - &  \textbf{3.3}        & 2.5             & 3.2       &  \textbf{3.6}                 &  4 \\
%     BC  & 0 (0) &  \textbf{0.47 (0.67)}        & \textbf{0.55 (0.67)}             & \textbf{0.60 (0.67)}       &  0.47 (0.67)                  &  0.53 (0.67) \\
%     %BC w/ dropout   & - &  2.1        & \textbf{3.5}            & 2.2       &  3.7                 &  2.6   \\
%     IRIS            & 0.08 (0.33) & 0.47 (0.67) & 0.45 (0.50) & 0.57 (0.67) & 0.53 (0.67) & 0.52 (0.67) \\
%     \bottomrule
% \end{tabular}
\end{table}

==> table/evaluation_one_leg_subtask.tex <==
\begin{table}[ht]
\centering
\caption{Subtask success rates of one-leg assembly task. \yw{numbers are random}}
\label{tab:evaluation_one_leg_subtask}    
\begin{tabular}{l|ccccc}
    \toprule
     & Tabletop & Placing  &  Leg     &  Inserting  &  Screwing    \\
    \midrule
    % Scripted Agent & 90\%  &  78\%        & 10\%            & 0\%       &  0\%                   \\
    BC             & 1.00 &  0.90   & 0.90      & 0.5     &  0.3    \\           
    BC-RNN         & 1.00 &  0.90   & 0.90      & 0.5     &  0.3    \\          
    IQL            & 1.00 &  0.90   & 0.90      & 0.5     &  0.3    \\         
    IRIS           & 1.00 &  0.90   & 0.90      & 0.5     &  0.3    \\          
    IBC            & 1.00 &  0.90   & 0.90      & 0.5     &  0.3    \\        
    BeT            & 1.00 &  0.90   & 0.90      & 0.5     &  0.3    \\
    \bottomrule
\end{tabular}
\end{table}

==> table/iql_hyperparams.tex <==
\begin{table}[ht]
  \caption{IQL hyperparameters.}
  \label{tab:hyperparameter_iql}
  \centering
  \begin{tabular}{ll}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Learning rate & 3e-4 \\ 
    Learning rate decay & Cosine decay \\
    \# Mini-batches & 256  \\
    Policy \# Hidden units &(512, 256, 256)  \\
    Q/V \# Hidden units &(512, 256, 256)  \\
    Activation & ReLU  \\
    Image encoder & R3M \\
    Reward discount factor ($\gamma$) & 0.996 \\
    Expectile ($\tau$) & 0.8 \\
    Inverse temperature ($\beta$) & 0.5 \\
    % Action normalization & True \\
    \bottomrule
  \end{tabular}
\end{table}
